Poncelet triangles: conic loci of the orthocenter and of the isogonal conjugate of a fixed point

We prove that over a Poncelet triangle family interscribed between two nested ellipses $\mathcal{E},\mathcal{E}_c$, (i) the locus of the orthocenter is not only a conic, but it is axis-aligned and homothetic to a $90^o$-rotated copy of $\mathcal{E}$, and (ii) the locus of the isogonal conjugate of a fixed point $P$ is also a conic (the expected degree was four); a parabola (resp. line) if $P$ is on the (degree-four) envelope of the circumcircle (resp. on $\mathcal{E}$). We also show that the envelope of both the circumcircle and radical axis of incircle and circumcircle contain a conic component if and only if $\mathcal{E}_c$ is a circle. The former case is the union of two circles!

==> 000_setup.tex <==
\usepackage{mathptmx}
%\setmainfont{TeX Gyre Termes}
%\setmathfont{TeX Gyre Termes Math}
\usepackage[margin=1.25in]{geometry}
\linespread{0.95}
\makeatletter
% Redefine \section to reduce spacing
%\def\section{\@startsection{section}{1}%
%  \z@{1.5ex \@plus 0.5ex \@minus 0.5ex}%
%  {1ex \@plus 0.2ex}%
%  {\normalfont\bfseries}}
%\makeatother

\usepackage{graphics}
\usepackage{thmtools}
\usepackage{wasysym}
%\usepackage{arxiv}
%\usepackage{enseign}
%\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{amsthm}
\usepackage{amsbsy,amsmath,amssymb,amscd,amsfonts}
\usepackage{xstring}
\usepackage[pagebackref=true]{hyperref}
\usepackage[nameinlink,capitalize,noabbrev]{cleveref}
%\usepackage{hyperref}
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography

\DeclareRobustCommand{\hrefs}[1]{%
  \def\temphrefsurl{#1}% Store the full URL
  \IfBeginWith{\temphrefsurl}{http://}{%
    \StrGobbleLeft{\temphrefsurl}{7}[\temphrefsdisplayurl]% Remove "http://" (7 chars)
  }{%
    \IfBeginWith{\temphrefsurl}{https://}{%
      \StrGobbleLeft{\temphrefsurl}{8}[\temphrefsdisplayurl]% Remove "https://" (8 chars)
    }{%
      % Fallback if neither http:// nor https:// is found
      \def\temphrefsdisplayurl{\temphrefsurl}% Display the full URL as is
    }%
  }%
  \href{\temphrefsurl}{\texttt{\temphrefsdisplayurl}}% Create the link
}

\usepackage{graphicx,float,latexsym,color}
\usepackage[export]{adjustbox}


%\usepackage{mathspec}
\usepackage[font={scriptsize,it},skip=5pt]{caption}
\newcommand{\zcaption}[1]{
\captionsetup{width=0.9\linewidth}\caption{#1}}
\usepackage{subcaption}
%\let\proof\relax
%\let\endproof\relax

\usepackage{makecell}
\renewcommand{\arraystretch}{1.2}

\usepackage[dvipsnames]{xcolor}

\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}
\hypersetup{
    %bookmarks=true,         % show bookmarks bar?
    %unicode=true,          % non-Latin characters in Acrobat’s bookmarks
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of 
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=OliveGreen,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=black,      % color of file links
    urlcolor=red           % color of external links
}

\usepackage{listings}
\usepackage{lineno}
\def\linenumberfont{\normalfont\small\sffamily}
%a4: 210 x 297
%\textwidth=125mm
%\textheight=195mm
\arraycolsep=2pt
\captionsetup{width=120mm}

\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\tb}[1]{\textbf{#1}}
%\newcommand{\tr}[1]{\tc{Red}{to do}}
\newcommand{\tr}[1]{\tc{Red}{#1}}
\newcommand{\ti}[1]{\textit{#1}}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
 
\usepackage{comment}
\usepackage{microtype}
\usepackage{footnote}
%\usepackage{tablefootnote}
%\usepackage{longtable}

%\usepackage{night}

\renewcommand{\O}{\mathcal{O}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\D}{\mathbb{D}}
\renewcommand{\T}{\mathcal{T}}
\newcommand{\Tt}{\T_{\triangle}}
\newcommand{\To}{\T_{\circ}}
\newcommand{\Et}{\E_{\triangle}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Rm}{\mathcal{R}}
\newcommand{\Cp}{\mathbb{C}}
\newcommand{\ol}{\overline}
\renewcommand{\l}{\lambda}
\newcommand{\X}{\mathcal{X}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\gP}{P^{\dagger}}
\newcommand{\gL}{\L^{\dagger}}

\newcommand{\torp}[2]{\texorpdfstring{#1}{#2}}
\newcommand{\ab}{_{\alpha,\beta}}
\newcommand{\rc}{\raisebox{0.3ex}{,}}
\newcommand{\rd}{\raisebox{0.3ex}{.}}

\usepackage{breqn}
\setlength{\mathindent}{0pt}
\renewcommand{\eqnumfont}{\normalfont}

\newcommand{\tightmath}[1]{%
  \begingroup
    \thinmuskip=0mu
    \medmuskip=0mu
    \thickmuskip=0mu
    #1%
  \endgroup
}
\setlength{\fboxsep}{0pt}  % Padding inside the frame

\newcommand{\twofigs}[4]{%
  \begin{figure}[htbp]
    \centering
    \fbox{%
      \begin{minipage}[c]{0.98\textwidth}
        \centering
        \hfill
        \begin{minipage}[c]{0.45\textwidth}
          \centering
          \vspace{5pt}
          \includegraphics[width=\linewidth]{#1}
          \vspace{0pt}
        \end{minipage}%
        \hspace{0.5em}
        \vrule width 0.5pt
        \hspace{0.5em}
        \begin{minipage}[c]{0.45\textwidth}
          \centering
          \vspace{5pt}
          \includegraphics[width=\linewidth]{#2}
          \vspace{0pt}
        \end{minipage}
        \hfill
      \end{minipage}
    }
    \caption{#3}
    \label{#4}
  \end{figure}
}

% does not work with cleveref
%\renewcommand{\cref}[1]{\ref{#1}}
%\usepackage{refcheck}

% alternative to refcheck, works with cleveref
%\usepackage[outer]{showlabels}
%\renewcommand{\showlabelfont}{\small\color{red}\ttfamily}


==> app/510_app_affine_triples.tex <==
\cref{tab:triples} lists the $\alpha,\beta,\gamma$ used to express a given triangle center $X_k$ as the linear combination $\alpha X_1+\beta X_2+\gamma X_3$, where $\rho=r/R$ (a more complete table appears in \cite[Table 1]{helman2021-theory}):

%\setlength{\tabcolsep}{2pt}
%\renewcommand{\arraystretch}{1.3}
% delete: 8, 9, 13, 14, 16, 17
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
%& $X_1$ & $X_2$ & $X_3$ & $X_4$ & $X_5$ & $X_7$ & $X_8$ & *$X_9$ & *$X_{10}$ & $X_{11}$ & $X_{12}$ & $X_{20}$ & *$X_{21}$ & *$X_{35}$ & $X_{36}$ & *$X_{40}$  & *$X_{46}$ \\ 
%\hline
%$\alpha$ & $1$ & $0$ & $0$ & $0$ & $0$ & $\frac{2\rho+4}{\rho+4}$ & $-2$ & *$\frac{-\rho-2}{\rho+4}$ & *$-\frac{1}{2}$ & $\frac{1}{1-2\rho}$ & $\frac{1}{1+2\rho}$ & $0$ & *$0$ & *$\frac{1}{2\rho+1}$ & $\frac{1}{1-2\rho}$ & *$-1$ & *$\frac{1+\rho}{1-\rho}$ \\
%\hline
%$\beta$ & $0$ & $1$ & $0$ & $3$ & $\frac{3}{2}$ & $\frac{3\rho}{\rho+4}$ & $3$ & $\frac{6}{\rho+4}$ & $\frac{3}{2}$ & $\frac{-3\rho}{1-2\rho}$ & $\frac{3\rho}{1+2\rho}$ & $-3$ & $\frac{3}{2\rho+3}$ & $0$ & $0$ & $0$   & $0$ 
%\\
%\hline
%$\gamma$ & $0$ & $0$ & $1$ & $-2$ & $-\frac{1}{2}$ & $\frac{-4\rho}{\rho+4}$ & $0$ & $\frac{2\rho}{\rho+4}$ & $0$ & $\frac{\rho}{1-2\rho}$ & $\frac{-\rho}{1+2\rho}$ & $4$ & $\frac{2\rho}{2\rho+3}$ & $\frac{2\rho}{2\rho+1}$ & $\frac{-2\rho}{1-2\rho}$ & $2$ 
% & $\frac{-2\rho}{1-\rho}$ \\ \hline 
% \end{tabular}

% gemini
\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& $X_1$ & $X_2$ & $X_3$ & $X_4$ & $X_5$ & $X_7$ & $X_8$ & $X_{11}$ & $X_{12}$ & $X_{20}$ & $X_{36}$ & $X_{80}$\\
\hline
$\alpha$ & $1$ & $0$ & $0$ & $0$ & $0$ & $\frac{2\rho+4}{\rho+4}$ & $-2$ & $\frac{1}{1-2\rho}$ & $\frac{1}{1+2\rho}$ & $0$ & $\frac{1}{1-2\rho}$ & $\frac{2\rho+1}{1-2\rho}$ \\
\hline
$\beta$ & $0$ & $1$ & $0$ & $3$ & $\frac{3}{2}$ & $\frac{3\rho}{\rho+4}$ & $3$ & $\frac{-3\rho}{1-2\rho}$ & $\frac{3\rho}{1+2\rho}$ & $-3$ & $0$ & $\frac{-6\rho}{1-2\rho}$ \\
\hline
$\gamma$ & $0$ & $0$ & $1$ & $-2$ & $-\frac{1}{2}$ & $\frac{-4\rho}{\rho+4}$ & $0$ & $\frac{\rho}{1-2\rho}$ & $\frac{-\rho}{1+2\rho}$ & $4$ & $\frac{-2\rho}{1-2\rho}$ & $\frac{2\rho}{1-2\rho}$ \\
\hline
\end{tabular}
\zcaption{Affine triples for triangle centers used in the text.}
\label{tab:triples}
\end{table}

%\vspace{.5 em}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
%& *$X_{55}$ & *$X_{56}$ & *$X_{57}$ & *$X_{63}$ & $X_{65}$ & $X_{72}$ & $X_{78}$ & $X_{79}$ & $X_{80}$ & $X_{84}$ & $X_{90}$ & $X_{100}$ & $X_{104}$ & $X_{119}$ \\ \hline
%$\alpha$ & $\frac{1}{1+\rho}$ & $\frac{1}{1-\rho}$ & $\frac{2+\rho}{2-\rho}$ & $\frac{-\rho-2}{\rho+1}$ & {\scriptsize $\rho+1$} & {\scriptsize $-\rho-2$} & $\frac{\rho+2}{\rho-1}$ & 1 & $\frac{2\rho+1}{1-2\rho}$ & $\frac{-\rho-2}{\rho}$ & $\frac{-(\rho+1)^2}{\rho^2+2\rho-1}$ & $\frac{2}{2\rho-1}$ & $\frac{-2}{2\rho-1}$ & $\frac{1}{2\rho-1}$ \\ \hline
%$\beta$ & $0$ & $0$ & $0$ & $\frac{3}{\rho+1}$ & $0$ & $3$ & $\frac{-3}{\rho-1}$ & $\frac{6\rho}{2\rho+3}$ & $\frac{-6\rho}{1-2\rho}$ & $\frac{6}{\rho}$ & $\frac{6\rho}{\rho^2+2\rho-1}$ & $\frac{-3}{2\rho-1}$ & $\frac{3}{2\rho-1}$ & $\frac{3\rho-3}{2\rho-1}$ \\ \hline
%$\gamma$ & $\frac{\rho}{1+\rho}$ & $\frac{-\rho}{1-\rho}$ & $\frac{-2\rho}{2-\rho}$ & $\frac{2\rho}{\rho+1}$ & {\small $-\rho$} & {\small $\rho$} & $0$ & $\frac{-6\rho}{2\rho+3}$ & $\frac{2\rho}{1-2\rho}$ & $\frac{2\rho-4}{\rho}$ & $\frac{2\rho(\rho-1)}{\rho^2+2\rho-1}$ & $\frac{2\rho}{2\rho-1}$ & $\frac{2\rho-2}{2\rho-1}$ & {$\frac{-\rho+1}{2\rho-1}$}\\ \hline
%\end{tabular}

%\vspace{.5 em}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
%\hline
%& $X_{140}$ & $X_{142}$ & $X_{144}$ & $X_{145}$ & $X_{149}$ & $X_{153}$ & $X_{165}$ & $X_{191}$ & $X_{200}$ \\ \hline
%$\alpha$ & $0$ & $\frac{\rho+2}{2\rho+8}$ & $\frac{-4\rho-8}{\rho+4}$ & $\frac{4}{7}$ & $\frac{-4}{6\rho-3}$ & $\frac{4}{6\rho-3}$ & $-\frac{1}{3}$ & $-1$ & $\frac{\rho+4}{\rho-2}$ \\ \hline 
%$\beta$ & $\frac{3}{4}$ & $\frac{3\rho+6}{2\rho+8}$ & $\frac{12-3\rho}{\rho+4}$ & $\frac{3}{7}$ & $\frac{-6\rho+9}{6\rho-3}$ & $\frac{-6\rho-3}{6\rho-3}$ & $0$ & $\frac{6}{2\rho+3}$ & $\frac{-6}{\rho-2}$ \\ \hline
%$\gamma$ & $\frac{1}{4}$ & $\frac{-2\rho}{2\rho+8}$ & $\frac{8\rho}{\rho+4}$ & $0$ & $\frac{12\rho-8}{6\rho-3}$ & $\frac{12\rho-4}{6\rho-3}$ & $\frac{4}{3}$ & $\frac{4\rho}{2\rho+3}$ & {$0$} \\ \hline
%\end{tabular}

%Notice $\alpha$,$\beta$,$\gamma$ are the same up to sign of $\rho$ for harmonic conjugate pairs ($X_{11}$,$X_{12}$), ($X_{35}$,$X_{36}$), ($X_{55}$,$X_{56}$).

